The Weakest Failure Detector for Genuine Atomic Multicast (Extended Version)

Atomic broadcast is a group communication primitive to order messages across a set of distributed processes. Atomic multicast is its natural generalization where each message $m$ is addressed to $dst(m)$, a subset of the processes called its destination group. A solution to atomic multicast is genuine when a process takes steps only if a message is addressed to it. Genuine solutions are the ones used in practice because they have better performance. Let $G$ be all the destination groups and $F$ be the cyclic families in it, that is the subsets of $G$ whose intersection graph is hamiltonian. This paper establishes that the weakest failure detector to solve genuine atomic multicast is $\mu=(\wedge_{g,h \in G}~\Sigma_{g \cap h}) \wedge (\wedge_{g \in G}~\Omega_g) \wedge \gamma$, where (i) $\Sigma_P$ and $\Omega_P$ are the quorum and leader failure detectors restricted to the processes in $P$, and (ii) $\gamma$ is a new failure detector that informs the processes in a cyclic family $f \in F$ when $f$ is faulty. We also study two classical variations of atomic multicast. The first variation requires that message delivery follows the real-time order. In this case, $\mu$ must be strengthened with $1^{g \cap h}$, the indicator failure detector that informs each process in $g \cup h$ when $g \cap h$ is faulty. The second variation requires a message to be delivered when the destination group runs in isolation. We prove that its weakest failure detector is at least $\mu \wedge (\wedge_{g, h \in G}~\Omega_{g \cap h})$. This value is attained when $F=\varnothing$.

==> Makefile <==
ALL=$(wildcard *.tex appendix/*.tex slides/*.tex slides/brief/*.tex)) 
BIB=$(wildcard *.bib)
MAIN=paper.tex
SLIDES=slides.tex
SLIDES-BRIEF=slides-brief.tex
LATEX=rubber --pdf --unsafe

BRIEF=brief
PDFLATEX=texfot pdflatex -file-line-error
IGNORE="(texfot: invoking: pdflatex|This is pdfTeX|Underfull|\\vspace should only be used to provide space above/below)"
BIB=bibtex

.DEFAULT_GOAL := all

all: ## Build full document
	$(LATEX) $(MAIN)                # main run

clean: ## Clean LaTeX and output figure files
	rubber --clean $(MAIN)
	rm -f $(FIGURES_PDF) $(FIGURES_PNG)

watch: ## Recompile on any update of LaTeX or SVG sources
	@while [ 1 ]; do;          \
	  inotifywait $(ALL);    \
	  sleep 0.01;            \
          make all;              \
          echo "\n----------\n"; \
          done

help:  # http://marmelab.com/blog/2016/02/29/auto-documented-makefile.html
	@grep -P '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-20s\033[0m %s\n", $$1, $$2}'


brief:
	@$(PDFLATEX) $(BRIEF).tex | grep -vE $(IGNORE)
	@$(BIB) $(BRIEF).aux
	@$(PDFLATEX) $(BRIEF).tex | grep -vE $(IGNORE)
	@$(PDFLATEX) $(BRIEF).tex | grep -vE $(IGNORE)

brief-sources:
	rm -rf /tmp/brief
	mkdir -p /tmp/brief/figures/brief
	cp brief.tex /tmp/brief
	cp abstract.tex /tmp/brief
	cp acmart.cls /tmp/brief
	cp brief.bib /tmp/brief
	cp format.sty /tmp/brief
	cp macros.sty /tmp/brief
	cp paper.sty /tmp/brief
	cp brief.bbl /tmp/brief
	cp Makefile /tmp/brief
	cp figures/brief/family.tex /tmp/brief/figures/brief
	tar -C /tmp -zcf brief.tar.gz brief
	rm -rf /tmp/brief

slides:
	${LATEX} ${SLIDES}

slides-brief:
	${LATEX} ${SLIDES-BRIEF}

arxiv-clean:
	rm -Rf arxiv/
	rm -f arxiv.tar.gz

arxiv: all
	mkdir -p arxiv/
	cp lipics-v2021.cls cc-by.pdf lipics-logo-bw.pdf orcid.pdf arxiv/
	cp Makefile arxiv/
	cp format.sty arxiv/
	cp macros.sty arxiv/
	cp paper.sty arxiv/
	cp paper.tex arxiv/
	cp abstract.tex arxiv/
	cp introduction.tex arxiv/
	cp problem.tex arxiv/
	cp candidate.tex arxiv/
	cp sufficiency.tex arxiv/
	cp necessity.tex arxiv/
	cp variations.tex arxiv/
	cp conclusion.tex arxiv/
	cp discussion.tex arxiv/
	cp appendix/model.tex arxiv/appendix-model.tex
	sed -i -e s/{appendix\\/model/{appendix-model/g arxiv/paper.tex 
	cp appendix/omega.tex arxiv/appendix-omega.tex
	sed -i -e s/{appendix\\/omega/{appendix-omega/g arxiv/paper.tex
	cp figures/recap.tex arxiv/figures-recap.tex
	sed -i -e s/{figures\\/recap/{figures-recap/g arxiv/introduction.tex
	cp figures/family.tex arxiv/figures-family.tex
	sed -i -e s/{figures\\/family/{figures-family/g arxiv/candidate.tex
	cp figures/fix.tex arxiv/figures-fix.tex
	sed -i -e s/{figures\\/fix/{figures-fix/g arxiv/sufficiency.tex
	cp figures/trivias.tex arxiv/figures-trivias.tex
	sed -i -e s/{figures\\/trivias/{figures-trivias/g arxiv/sufficiency.tex
	cp figures/gamma.tex arxiv/figures-gamma.tex
	sed -i -e s/{figures\\/gamma/{figures-gamma/g arxiv/necessity.tex
	cp figures/critical.tex arxiv/figures-critical.tex
	sed -i -e s/{figures\\/critical/{figures-critical/g arxiv/appendix-omega.tex
	cp figures/gadget.tex arxiv/figures-gadget.tex
	sed -i -e s/{figures\\/gadget/{figures-gadget/g arxiv/appendix-omega.tex
	cp algorithms/sufficiency.tex arxiv/algorithms-sufficiency.tex
	sed -i -e s/{algorithms\\/sufficiency/{algorithms-sufficiency/g arxiv/sufficiency.tex
	cp algorithms/sigma.tex arxiv/algorithms-sigma.tex
	sed -i -e s/{algorithms\\/sigma/{algorithms-sigma/g arxiv/necessity.tex
	cp algorithms/gamma.tex arxiv/algorithms-gamma.tex
	sed -i -e s/{algorithms\\/gamma/{algorithms-gamma/g arxiv/necessity.tex
	cp algorithms/indicator.tex arxiv/algorithms-indicator.tex
	sed -i -e s/{algorithms\\/indicator/{algorithms-indicator/g arxiv/variations.tex
	cp algorithms/omega.tex arxiv/algorithms-omega.tex
	sed -i -e s/{algorithms\\/omega/{algorithms-omega/g arxiv/appendix-omega.tex
	cp paper.bib arxiv/
	cp paper.bbl arxiv/
	cp bib.bib arxiv/
	cp plainurl.bst arxiv/
	tar -C arxiv -zcf arxiv.tar.gz .
	rm -Rf arxiv/

dagstuhl:
	mkdir -p dagstuhl/
	cp lipics-v2021.cls cc-by.pdf lipics-logo-bw.pdf orcid.pdf dagstuhl/
	cp Makefile dagstuhl/
	cp format.sty dagstuhl/
	cp macros.sty dagstuhl/
	cp paper.sty dagstuhl/
	cp paper.tex dagstuhl/
	sed -i 's/\\longversiontrue/\\longversionfalse/g' dagstuhl/paper.tex
	cp abstract.tex dagstuhl/
	cp introduction.tex dagstuhl/
	cp problem.tex dagstuhl/
	cp candidate.tex dagstuhl/
	cp sufficiency.tex dagstuhl/
	cp necessity.tex dagstuhl/
	cp variations.tex dagstuhl/
	cp conclusion.tex dagstuhl/
	cp discussion.tex dagstuhl/
	cp figures/recap.tex dagstuhl/figures-recap.tex
	sed -i -e s/{figures\\/recap/{figures-recap/g dagstuhl/introduction.tex
	cp figures/family.tex dagstuhl/figures-family.tex
	sed -i -e s/{figures\\/family/{figures-family/g dagstuhl/candidate.tex
	cp algorithms/sufficiency.tex dagstuhl/algorithms-sufficiency.tex
	sed -i -e s/{algorithms\\/sufficiency/{algorithms-sufficiency/g dagstuhl/sufficiency.tex
	cp algorithms/sigma.tex dagstuhl/algorithms-sigma.tex
	sed -i -e s/{algorithms\\/sigma/{algorithms-sigma/g dagstuhl/necessity.tex
	cp algorithms/gamma.tex dagstuhl/algorithms-gamma.tex
	sed -i -e s/{algorithms\\/gamma/{algorithms-gamma/g dagstuhl/necessity.tex
	cp algorithms/indicator.tex dagstuhl/algorithms-indicator.tex
	sed -i -e s/{algorithms\\/indicator/{algorithms-indicator/g dagstuhl/variations.tex
	cp paper.bib dagstuhl/
	cp bib.bib dagstuhl/
	cp plainurl.bst dagstuhl/
	tar -C dagstuhl -zcf dagstuhl.tar.gz .
	rm -Rf dagstuhl

.PHONY: help


